Comparison of control regularization techniques for minimum-fuel low-thrust trajectory design using indirect methods

Minimum-fuel low-thrust trajectories typically consist of a finite, yet unknown number of switches in the thrust magnitude profile. This optimality-driven characteristic of minimum-fuel trajectories poses a challenge to the numerical methods that are typically used for solving the resulting Hamiltonian boundary-value problems (BVPs). In this paper, we compare the impact of the popular hyperbolic-tangent-based smoothing with a novel L2-norm-based smoothing on the convergence performance of quasi-Newton gradient-based methods. Both smoothing methods are applied directly at the level of control, which offer a significant implementation simplicity. We also investigate the application of each method in scenarios where the State Transition Matrix (STM) is used for accurate calculation of the sensitivities of the residual vector of the resulting BVPs with respect to the unknown initial costate values. The effectiveness of each control smoothing method is assessed across several benchmark minimum-fuel low-thrust trajectory optimization problems.

==> CR3BP.tex <==
\subsection{Problem 2: Low-Thrust Trajectories in Restricted Three-Body Problem Dynamic Model}
We consider now the problem of designing low-thrust trajectories in the restricted three body (R3B) dynamic model. The R3B of the Earth-moon system is of particular interest due to the existence of periodic orbits at the so-called Lagrangian (libration) points. Assuming a rotating frame, the existence of these points is due to the combined gravitational pull of the primaries (the Earth and Moon) along with the acceleration due to the rotation of the frame. As it is well-known, five stationary (libration) points exist with zero velocity and zero acceleration with respect to the rotating frame. Moreover, it is possible to find closed periodic orbits in the vicinity of these points. These  can be used as quasi-stable orbits for any spacecraft (with station-keeping, of course). What makes these orbits appealing is the fact that the amount of propellant required for keeping a spacecraft in these orbits is relatively small and, in some cases, these orbits are very advantageous for cis-lunar navigation and communications. These orbits can also be used for observation purposes or be used for establishment of space outposts beyond low-Earth orbits. 

In particular, we study the problem of transferring a spacecraft from a geostationary transfer orbit (GTO) to a halo orbit around the L1 point of the Earth-moon system. Halo orbits are periodic, three-dimensional orbits near L1, L2 or L3 Lagrange points. It is also possible to transfer a spacecraft between L1 and L2 points of the Earth-moon system. While we have not presented the solution to this problem in this paper, it is possible to design transfer trajectories between libration points of the Earth-moon system to their counterparts in the Sun-Earth R3B system. A spacecraft placed in an orbit around the L1 point of the Sun-Earth system can, for example, serve as an early-warning system for Solar flares that may disrupt digital communications. There are a number of potential applications that makes orbits around these points particularly attractive for future space missions. 

On the other hand, the design of low-thrust trajectories to halo orbits are challenging due to the following factors: 1) the time of transfer is usually long, 2) many revolutions are usually required, and 3) the force field of the three-body dynamical model is highly nonlinear. It is shown that for minimum-fuel trajectories, the control input has a bang-off-bang behavior with multiple switches between coasting and thrusting control arcs. We utilize the tangent hyperbolic function that we introduced in the previous section. 

Over the past 200 years, a great number of scholars have devoted their life to analyze and study the motion of objects in the dynamic model of R3Bs. A special sets of units, and coordinate frames for this problem have been found useful to normalize the system and makes its analysis simpler. The dynamics is usually written in a co-rotating frame where the masses of the Earth and Moon are $1-\mu$ and $\mu$, respectively. The unit of mass is the sum of the two masses, i.e., $m_1 + m_2 = 1$. The time unit is chosen such that the gravitational constant $G = 1$ is absorbed into a new time unit (TU), which results in a unit angular velocity, i.e., $\omega = 1$ rad/TU. The system parameters are scaled such the one Length Unit (LU) is equal to the distance from the Earth to the moon. 

Let $\bm{x}^{\top} = [\bm{r}^{\top},\bm{v}^{\top},m]$ denote the state vector, where $\bm{r}^{\top}  = [x,y,z]$, and $\bm{v}^{\top} = [v_x,v_y,v_z]$ are position and velocity vectors, respectively, and $m$ is the mass of the spacecraft. For low-thrust trajectories, the equations of motions can be written as,
\begin{align}
\dot{\bm{x}} = \bm{f}(\bm{x},\bm{u},\delta) = \begin{bmatrix}
\dot{\bm{r}}\\
\dot{\bm{v}}\\
\dot{m}
\end{bmatrix} = \begin{bmatrix}
\bm{v}\\
\bm{g}(\bm{r}) + \bm{h}(\bm{v})+\frac{T_{\text{max}}}{m}\delta \bm{u}\\
-\frac{T_{\text{max}}}{c} \delta
\end{bmatrix}.
\end{align}
Similar to the previous problem, the control thrust vector is expressed in terms of a unit vector, $\bm{u}$, and an engine throttle factor, $\delta$. The functions $\bm{g}(\bm{r})$ and $\bm{h}(\bm{v})$ are defined as
\begin{align}
\bm{g}(\bm{r}) = & \begin{bmatrix}
x-\frac{(1-\mu)(x+\mu)}{r^3_1} -  \mu\frac{x+\mu-1}{r^3_2}\\
y - \frac{1-\mu}{r^3_1}y-  \mu\frac{y}{r^3_2}\\
-\frac{1-\mu}{r^3_1}z-  \mu\frac{z}{r^3_2}
\end{bmatrix}, \\
\bm{h}(\bm{v}) = & \begin{bmatrix}
2v_y\\
-2v_x\\
0
\end{bmatrix},
\end{align}
where $r_1 = \sqrt{(x+\mu)^2+y^2+z^2}$ and $r_2 = \sqrt{(x+\mu-1)^2+y^2+z^2}$ denote the distances of the spacecraft from the Earth and Moon, respectively. 

Now, formulation of the minimum-fuel problem is presented. The cost functional is identical to the one defined in Eq.~\eqref{eq:costp1}. We proceed by forming the Hamiltonian as
\begin{align} \label{eq:HamilMinTime}
H = \frac{T_{\text{max}}}{c} \delta+ \bm{\lambda}_{\bm{r}}^{\top}  \bm{v} + \bm{\lambda}_{\bm{v}}^{\top} \left [\bm{g}(\bm{r}) + \bm{h}(\bm{v}) + \frac{T_{\text{max}}}{m} \delta \hat{\bm{u}} \right ] - \lambda_m \frac{T_{\text{max}}}{c} \delta,
\end{align}
where $\bm{\lambda}^{\top} = [\bm{\lambda}^{\top}_{\bm{r}}, \bm{\lambda}^{\top}_{\bm{v}}, \lambda_m]$. The next step is to derive the costates differential equations,
\begin{align} \label{eq:costatedyanmicsR3BP}
\dot{\bm{\lambda}} = -\frac{\partial H}{\partial \bm{x}} = \begin{bmatrix}
\dot{\bm{\lambda}}_{\bm{r}} \\
\dot{\bm{\lambda}}_{\bm{v}} \\
\dot{\lambda}_m
\end{bmatrix} = \begin{bmatrix}
                  - \bm{G}^T \bm{\lambda}_{\bm{v}} \\
                  -\bm{\lambda}_{\bm{r}} - \bm{H}^T \bm{\lambda}_{\bm{v}} \\
                  \frac{T_{\text{max}}}{m^2} \bm{\lambda}^{\top}_{\bm{v}}  \delta \bm{u}
                \end{bmatrix},
\end{align}
where $\bm{G} = \partial \bm{g}(\bm{r})/\partial \bm{r}$ and $\bm{H} = \partial \bm{h}(\bm{v})/\partial \bm{v}$. Appendix B lists all the non-zero elements of $\bm{G}$ and $\bm{H}$.

Let $\bm{p}$ denote the primer vector defined as the negative of the co-state vector associated with the velocity vector, $\bm{p} = -\bm{\lambda}_{\bm{v}}$. The extremal direction of the control vector, $\bm{u}$ can be determined as 
\begin{equation} \label{eq:extremaldirection}
\bm{u}^* = \frac{\bm{p}}{||\bm{p}||}.
\end{equation}
If Eq.~\eqref{eq:extremaldirection} is substituted for the unit vector $\bm{u}$ in Eq.~\eqref{eq:HamilMinTime}, the Hamiltonian can be written as
\begin{align} \label{eq:HamilMinTimeUsub}
H = H_0 - \frac{T_{\text{max}}}{c} \left [ \frac{c \lambda_v}{m} + \lambda_m -1 \right ] \delta, 
\end{align}
where $H_0$ denotes the terms that do not include the throttling input. The sign of the bracket term is the critical issue and it is convenient to define the bracket as the switching function, 
\begin{equation} \label{eq:sfR3BP}
S = \frac{c \lambda_v}{m} +\lambda_m -1.
\end{equation}
The optimal value of the throttling input is determined by using PMP, i.e., the control input should minimize the Hamiltonian assuming that all of the other variables are fixed [\cite{longuski2014optimal}]. Assuming no singular arc, the following relation exists
\begin{align}
\delta^*(S)  = \begin{cases}
1&\text{for}~S>0, \\
0&\text{for}~S<0,
\end{cases} = \frac{1}{2} \left [ 1 + \text{sign}(S)\right].
\end{align}

The transversality conditions leads to $\lambda_m(t_f) = 0$ since final mass is a free variable. In addition, if Eq.~\eqref{eq:extremaldirection} is substituted in Eq.\eqref{eq:costatedyanmicsR3BP}, the time rate of change of the costate associated with mass is always non-positive
\begin{equation}
\dot{\bm{\lambda}}_m = -\frac{T_{\text{max}}}{m^2} \lambda_v \delta .
\end{equation}

Therefore, $\lambda_m(t_0) \geq 0$, which provides further information for its valid initial values. For a fixed-time rendezvous problem, the boundary conditions can be written in the form of seven equality constraints,
\begin{equation}\label{eq:posvelconp2}
\bm{\psi}(\bm{x}(t_f),t_f) =
\begin{bmatrix}
\bm{r}(t_f) - \bm{r}_T \\
\bm{v}(t_f) - \bm{v}_T \\
\lambda_m(t_f)
\end{bmatrix} = \bm{0},
\end{equation}
where $\bm{r}_T$ and $\bm{v}_T$ denote the position and velocity vectors, respectively, of the target point. The smoothed control input takes the following form
\begin{equation} \label{eq:smoothedthrottleR3BP}
\delta^*(S) = \frac{1}{2} \left [ 1+ \text{sign}(S) \right ] \cong \delta^*(S,\rho) = \frac{1}{2} \left [ 1+ \tanh \left ( \frac{S}{\rho} \right ) \right ],
\end{equation}
where $S$ denotes the switching function of the minimum-fuel formulation, Eq.~\eqref{eq:sfR3BP}. Let $\bm{z}^{\top} = [\bm{x}^{\top},\bm{\lambda}^{\top}]$ denote the state-costate vector, then, we can write,
\begin{equation*}
\dot{\bm{z}} = \bm{F} = \begin{bmatrix}
\dot{\bm{x}}\\
\dot{\bm{\lambda}}
\end{bmatrix},
\end{equation*}
where $\bm{u} = \hat{\bm{u}}^*$ and $\delta = \delta^*(S,\rho)$. Once, these values are substituted into $\bm{F}$, the equations of motions can be integrated implicitly. Altogether, the TPBVP of the minimum-fuel problem in the R3B can be written as finding the seven elements of the initial costate vector $\bm{\lambda}(t_0)$ to satisfy the seven dimensional terminal constraint vector function of Eq.~\eqref{eq:posvelconp2}. Notice $\bm{z}(t_f) = \bm{z}(\bm{x}(t_0), \bm{\lambda}(t_0))$. The resulting TPBVP consists of seven unknowns, $\bm{\lambda}(t_0)$ that constitute the vector of design variables and seven terminal constrains defined in Eq.~\eqref{eq:posvelconp2} . 
